Impact of Random Failures and Attacks on Poisson and Power-Law Random Networks

It appeared recently that the underlying degree distribution of networks may play a crucial role concerning their robustness. Empiric and analytic results have been obtained, based on asymptotic and mean-field approximations. Previous work insisted on the fact that power-law degree distributions induce high resilience to random failure but high sensitivity to attack strategies, while Poisson degree distributions are quite sensitive in both cases. Then, much work has been done to extend these results. We aim here at studying in depth these results, their origin, and limitations. We review in detail previous contributions and give full proofs in a unified framework, and identify the approximations on which these results rely. We then present new results aimed at enlightening some important aspects. We also provide extensive rigorous experiments which help evaluate the relevance of the analytic results. We reach the conclusion that, even if the basic results of the field are clearly true and important, they are in practice much less striking than generally thought. The differences between random failures and attacks are not so huge and can be explained with simple facts. Likewise, the differences in the behaviors induced by power-law and Poisson distributions are not as striking as often claimed.

==> courbes-conclu.tex <==
\newcommand{\courbeconclu}[3]{
\begin{figure}[!h]
\centering
\includegraphics[scale=0.42]{#1.sommets.fig.eps}
\ \ \ \ \ \ 
\includegraphics[scale=0.42]{#1.aretes.fig.eps}
\caption{Size of the largest connected component of #2 networks with #3,
as a function of the fraction of removed nodes or links by all
the strategies we have studied.}
\label{fig_#1_cc}
\end{figure}
}


\courbeconclu{er_10000_1.4}{Poisson}{average degree $1.4$}
\courbeconclu{er_10000_1.6}{Poisson}{average degree $1.6$}
\courbeconclu{er_10000_1.9}{Poisson}{average degree $1.9$}
\courbeconclu{er_10000_2.5}{Poisson}{average degree $2.5$}
\courbeconclu{sf_10000_2.5}{continuous power-law}{exponent $2.5$}
\courbeconclu{sf_10000_3}{continuous power-law}{exponent $3$}
\courbeconclu{vsf_10000_2.5}{discrete power-law}{exponent $2.5$}
\courbeconclu{vsf_10000_3}{discrete power-law}{exponent $3$}



==> nouveau.tex <==
\subsection{Towards a more realistic modeling}

Modeling large networks is a complex task and many parameters have to
be taken into account.
The approach to modeling we follow in this paper relies on {\em random sampling}:
given a set of properties of a real network that one wants to reproduce,
the goal is to choose with uniform probability a graph among the set of all
graphs having these properties.
This approach has the advantage of allowing to study precisely the impact of
a given property: if a certain behavior is observed on graphs obtained with
such a model, then we can conclude that this behavior is a consequence of
the studied property.
This type of model is also well-suited for exact proofs.
However, it also suffers from limitations:
some properties cannot currently be reproduced by this type of models.
It is for instance currently impossible to sample a graph uniformly at random
among all graphs having a given clustering coefficient, 
or even a given number of triangles.
In summary, this type of model is well-adapted for understanding and formal
proofs of the impact of some properties,
but is not currently able to reproduce all properties of real-world networks.

In this paper, we focus on the degree distribution of graphs,
and use models producing random graphs with given degree distributions.
However, the sole degree distribution
cannot reproduce the complexity of networks
(for instance it is  possible to
produce completely different networks having the exact same degree
distribution).
It has also been shown that when the sole
degree distribution is taken into account, high degree nodes tend be
connected to each other, which might not be
realistic~\cite{Doyle05robust}.

Efforts have therefore been made to study other properties and incorporate
them into random models.
For instance, scientists have studied
the assortativity
parameter~\cite{Newman2002AssortativeMixing}, the degree
correlations~\cite{Boguna2003EpidemiCorrelations,Vazquez2003ResilienceCorrelations}
where the probability $P(d|d')$ that a node of degree $d$ is linked to
another node of degree $d'$, or by the s(g) described
in~\cite{Doyle05robust,Li06towards} parameter which is the the sum of
$d_id_j$ for all links $(i,j)$, normalized by the larger value
obtainable on a graph with the same degree sequence. 

%To allow more realism, two orthogonal approaches exists: the first one consists in adding more constraints on the class of graph that are considered, for instance to take degree correlations into account, while the second approach is to use more realistic models based on observed constraints.

\noteperso{Mettre le paragraphe ci-dessous \`a la fin,
dans une partie ph\'enom\`enes ?}

In~\cite{Boguna2003EpidemiCorrelations}, the authors study the propagation of diseases on networks with degree correlations. The main conclusion is that correlations does not prevent epidemics from propagating. In a similar fashion, \cite{Vazquez2003ResilienceCorrelations} study the resilience of failures for assortative networks (nodes are linked to similar nodes) or disassortative networks. The resilience depends on the second moment of the degree distribution and the correlations: assortative networks are much resilient even with a finite second moment of the degree distribution, while disassortative networks can be fragile with a divergent second moment.

\medskip

%However, imposing more restrictions on the networks might not solve
%the problem of realism of these networks. 

Another, and orthogonal, approach consists of
taking into account properties that play a role in the construction
of a network.
For instance, in the case of the internet,
one can consider the way routers work,
or other technological or economic constraints. 
One then applies a construction process which respects the observed property and
produces in the end a graph similar to the original network.

The HOT, or {\em Heuristically Optimal Topology} or {\em Highly Optimized/Organized
Tolerance/Tradeoffs} framework belongs to this approach.

This type of approach has the advantage of being able to take into
account many properties that cannot be considered in random modeling.
This makes it relevant for producing graphs for simulation purposes.
However, the construction rules in these models create graph structures
that are hard to characterize, and in the end the properties of the
obtained graphs are not always fully understood.
A simple example of this is the preferential attachement model~\cite{barabasi99emergence},
which produces trees (if each new node creates a single link)
or graphs with no nodes of degree one (if new nodes create more than one link).
These models therefore allow to study the impact of the construction rule
on the observed behaviors,
but do not allow yet to study the impact of some topological properties of the networks.
Also, in the case of optimization models, it is not always easy
to find interesting parameters to optimize as it can be done for the
case of the Internet. Indeed performance related measures are quite
natural in the context of computer networks but can be harder to find
in social networks for instance.
In summary, this approach is relevant for taking into account complex network
properties, and for simulation purposes, but does not allow to study precisely
the impact of global topological properties.
Therefore, these two types of approachees are complementary.


%considering real characteristics of complex
%networks. 
The HOT framework has been mainly used in the context of the
Internet~\cite{Doyle05robust,Li04first}.
% but could be applied in many
%other contexts.
The authors of these papers propose to rewire a network with a given
degree distribution in a non random fashion which preserves the degree
sequence. The nonrandomness consists of rewiring with the aim of
optimizing some properties of the networks to mimic real properties:
technological, economic, etc. This kind of optimization can also be
found in the context of biological systems~\cite{Doyle08reverse}.

%This framework is very general and is referred as HOT, for .
%In general, random graphs generated this way are much more efficient, as defined below.


\medskip
Concerning network robustness, we only consider here the size of the largest
component as an indication of the state of the network after failures or attachks. This is used
since it describes the ability of nodes to communicate. However other
approaches have been introduced.

In~\cite{Latora2001Efficient,Holme2002Vulnerability} the authors use the efficiency, also called average inverse geodesic length, which is computed as $1/(N(N-1))\sum_{i,j}1/d_{ij}$, where $d_{ij}$ is the distance between $i$ and $j$. An high efficiency means that pairs of nodes are on average close to each other. This is very similar to the average distance but allows to consider disconnected networks, which is pertinent in our context.
In a similar fashion, the authors of~\cite{park03static} introduce the Diameter-Inverse-K (DIK) measure defined as $d/K$, where $d$ is the average distance between pairs of connected nodes, and $K$ is the fraction of pairs of nodes which are connected. It allows to take into account disconnected graphs and for connected graphs allows to distinguish between short or large average distance.
In~\cite{Crucitti2003EfficiencyScale-Free}, the authors consider that considering shortest paths can put a higher load on some nodes and that this load can increase when failures or attacks occurs. In consequence, each node is associated with a given capacity that cannot be exceeded without a lost of efficiency of the node, which increases the distances. This concept used with the efficiency of the network defined above has mainly been used for cascading failures and attacks but could be used as a more evolved definition of efficiency.

More specific measures have also been introduced. In particular, in the case of the Internet, nodes and links are used to carry some demand and the efficiency of the network can be measured as its capacity at carrying it. In~\cite{Li04first,Doyle05robust}, the authors define the maximal throughput based on the bandwidth of nodes, a routing matrix and the traffic demand for all nodes. In the case of the Internet, high degree nodes are at the periphery of the network and the fragility of the network lies more on the low degree core nodes that on the high degrees periphery nodes.

Some attack strategies based on
these measures of importance have also been introduced.
For instance, attack strategies that focus on important nodes rather than
on large degree nodes.
In~\cite{Holme2002Vulnerability} for instance, the authors
compare the removal of highest degree nodes with the removal of
highest betweenness nodes. Furthermore, the order of removal can be
either chosen before any removal occurs, or recalculated after each
removal, if the degree or betweenness of nodes has changed.

\medskip

We presented here a quick overview of the different types of graph modeling
that exist in the litterature, together with a brief discussion on their
advantages and drawback.
We also presented other attack or failures strategies, as
well as other definitions of network resilience.
Studying all this in detail is however out of the scope of this paper.

%The domain of the resilience of graphs to failures and attacks is therefore much larger than what will be investigated in the rest of this paper. While all these approaches are really interesting and challenging, it is not so easy to have a clear understanding of the phenomenon under concern, even with simple parameters for the graphs and the impact the removal can produce. 
